Constant Memory Attention Block

Modern foundation model architectures rely on attention mechanisms to effectively capture context. However, these methods require linear or quadratic memory in terms of the number of inputs/datapoints, limiting their applicability in low-compute domains. In this work, we propose Constant Memory Attention Block (CMAB), a novel general-purpose attention block that computes its output in constant memory and performs updates in constant computation. Highlighting CMABs efficacy, we introduce methods for Neural Processes and Temporal Point Processes. Empirically, we show our proposed methods achieve results competitive with state-of-the-art while being significantly more memory efficient.

==> core/04_relatedwork.tex <==

\section{Related Work} \label{sec:related_work}

NPs have used various methods to encode the context dataset. For example, CNPs~\citep{garnelo2018conditional} encode the context set via a deep sets encoder, ConvCNPs~\citep{gordon2019convolutional} use convolutions to build in translational equivariance.
Recent work~\citep{bruinsma2023autoregressive} builds on CNPs and ConvCNPs by proposing to make them autoregressive at deployment. 
ANPs~\citep{kim2019attentive}, LBANPs~\citep{feng2023latent}, and TNPs~\citep{nguyen2022transformer} use various kinds of attention to tackle underfitting. 
NP~\citep{garnelo2018neural} proposes to encode functional stochasticity in a latent variable.
NPs have found a wide-range of applications which include and are not limited to Temporal Point Processes~\citep{bae2023meta}, sequence data~\citep{singh2019sequential, willi2019recurrent}, modelling stochastic physics fields~\citep{holderrieth2021equivariant}, robotics~\citep{chen2022meta, li2022category}, and climate modeling~\citep{vaughan2021convolutional}.
For an in-depth overview, we refer the reader to the recent survey work~\citep{jha2022neural} on Neural Processes and their applications.


Transformers~\citep{vaswani2017attention} have achieved a large amount of success in a wide range of applications. 
However, the quadratic scaling of Transformers limits their applications to settings with but the quadratic scaling in terms of the number of inputs due to its self-attention layers renders it inapplicable to settings with large amounts of inputs e.g., images. 
There have been many proposed approaches to obtain efficiency gains such as sparse attention~\citep{huang2019ccnet} and low-rank self-attention~\citep{wang2020linformer}.
Closest to our work, several works~\citep{goyal2021coordination, jaegle2021perceiver, lee2019set} have proposed to use latent bottlenecks.
Set Transformers and related works~\citep{goyal2021coordination, lee2019set} utilises cross-attention to map the input array back and forth between an array with fewer elements to achieve a sub-quadratic complexity.
Perceiver~\citep{jaegle2021perceiver} utilises an asymmetric cross-attention method to distill the input array into a lower-dimensional latent bottleneck; after which, standard Transformer blocks are then applied to the latent space.
To the best of our knowledge, we are the first to propose an attention mechanism with an efficient update mechanism that allows for computing the output of the attention block in constant memory. 
For an in-depth overview, we refer the reader to the recent survey works~\citep{khan2022transformers,lin2022survey} on Transformers and their applications.

